CoCoGen: Physically-Consistent and Conditioned Score-based Generative Models for Forward and Inverse Problems

Recent advances in generative artificial intelligence have had a significant impact on diverse domains spanning computer vision, natural language processing, and drug discovery. This work extends the reach of generative models into physical problem domains, particularly addressing the efficient enforcement of physical laws and conditioning for forward and inverse problems involving partial differential equations (PDEs). Our work introduces two key contributions: firstly, we present an efficient approach to promote consistency with the underlying PDE. By incorporating discretized information into score-based generative models, our method generates samples closely aligned with the true data distribution, showcasing residuals comparable to data generated through conventional PDE solvers, significantly enhancing fidelity. Secondly, we showcase the potential and versatility of score-based generative models in various physics tasks, specifically highlighting surrogate modeling as well as probabilistic field reconstruction and inversion from sparse measurements. A robust foundation is laid by designing unconditional score-based generative models that utilize reversible probability flow ordinary differential equations. Leveraging conditional models that require minimal training, we illustrate their flexibility when combined with a frozen unconditional model. These conditional models generate PDE solutions by incorporating parameters, macroscopic quantities, or partial field measurements as guidance. The results illustrate the inherent flexibility of score-based generative models and explore the synergy between unconditional score-based generative models and the present physically-consistent sampling approach, emphasizing the power and flexibility in solving for and inverting physical fields governed by differential equations, and in other scientific machine learning tasks.

==> 05_fieldinversion.tex <==
\section{Field Reconstruction and Inversion with Sparse Measurements}\label{sec:fieldinversion}

Solving the reverse SDE can also be influenced by some conditioning variables $c$ in order to guide the final samples towards a sample from $p(x|c)$ rather than $p(x)$. We will not discuss the general case here, but rather we discuss a specific case of data imputation. Data imputation involves attempting to reconstruct a full data sample from partial measurements.

Consider a case in which pressure measurements are taken at some spatial locations in which the fluid flow is governed by Darcy flow. With few measurements, the goal is not only to reconstruct the rest of the pressure field, but also to reconstruct the entire permeability field. Thus, in the limit of measuring pressure on the entire spatial domain, predicting the permeability field becomes an inverse problem. 

We perform data imputation by first following the ideas in~\cite{song2021scorebased} in which $\Omega(x)$ denotes the known (measured) dimensions of $x$ and $\bar{\Omega(x)}$ denotes the unknown dimensions of x. Further, $f_{\bar{\Omega}}(\cdot, t)$ and $g_{\bar{\Omega}}(\cdot, t)$ define a restriction of the operators $f(\cdot, t)$ and $g(\cdot, t)$ in the SDE to the unknown dimensions only. 

As some portion of $x$ is known, a new diffusion process is defined such that $z(t) = \bar{\Omega}(x(t))$ and
\[
dz = f_{\bar{\Omega}}(z, t)dt + g_{\bar{\Omega}}(z, t)dw \; .
\]
However, we do not desire to simply sample from $p(z(t=0))$, but rather $p(z(t=0)|\Omega(x(t=0))=y)$, where $y$ are the measured values. The reverse process is therefore defined as
\[
dz = [f_{\bar{\Omega}}(z, t) - g_{\bar{\Omega}}(z, t)^2\nabla_z \log p_t(z|\Omega(x(0))=y)]dt + g_{\bar{\Omega}}(z, t)dw
\]
In is shown in~\cite{song2021scorebased} that $\nabla_z \log p_t(z|\Omega(x(0))=y)$ can be approximated by $\nabla_z \log p_t(u(t))$ where $u(t) = [z(t); \hat{\Omega}(x(t))]$ is a vector such that $\Omega(u(t)) = \hat{\Omega}(x(t))$ and $\bar{\Omega}(u(t)) = z(t)$. The quantity $\hat{\Omega}(x(t))$ denotes a random sample from $p_t(\Omega(x(t))|\Omega(x(0))=y)$, which can typically be obtained by sampling the corresponding dimensions from the forward SDE process. Thus, an approximation to $\nabla_z \log p_t(z|\Omega(x(0))=y)$ can be computed by leveraging the score function approximation $s_\theta(x(t), t)$ without any additional special training by sampling the known dimensions of $x(t)$ at each time step according to the forward process to approximately condition on the measured quantities. 

It is worth mentioning that performing data imputation in this manner can be orders of magnitude more expensive when solving the PF ODE reverse process rather than the reverse SDE process. It is illustrated in Sec.~\ref{sec:physical_consistency} that solving the PF ODE reverse process results in improved residual minimization with smaller cost when compared to the reverse SDE. However, as the outlined method of data imputation requires sampling from the forward process, sampling from the forward PF ODE process requires solving the PF ODE forward in time. In contrast, the forward SDE has a closed form solution to obtain samples at any given time, rendering it far more feasible and inexpensive to sample from $p_t(\Omega(x(t))|\Omega(x(0))=y)$.

We use the same score-based generative model defined in the experiments of~\ref{sec:physical_consistency} here. However, only the reverse SDE is solved. First, we perform the baseline data imputation approximation for various number of measurements. We define the number of measurements as $m$, and randomly select $m$ spatial locations to measure pressure in the physical domain. The random seed is kept constant such that for two cases in which $m_2 > m_1$, the spatial locations of case 1 are a subset of the spatial locations of case 2. 

For each experiment, we vary only the number of pressure measurements used to reconstruct the pressure field and invert the permeability field. The reverse process uses an Euler-Maruyama time integration method to solve the reverse SDE with 2,000 time steps. We also use $N=50$ physical consistency steps and $M=10$ additional physical consistency steps. For this experiment, we use both data with $s-16$ and $s=256$ dimensions. Pressure data is denoted $P$ with reconstructions denoted $\hat{P}$. Similarly, permeability data and reconstructions are denoted $K$ and $\hat{K}$ respectively. Tables~\ref{tab:reconstruction_darcy_n16} and~\ref{tab:reconstruction_darcy_n256} and Fig.~\ref{fig:reconstruction_darcy_base_n16} illustrate the results of this experiment.

\begin{table}[!htb]
\centering
\caption{Physical field reconstruction and field inversion with various number of pressure measurements (Darcy Flow, $s=16$).}
\label{tab:reconstruction_darcy_n16}
\begin{tabularx}{\textwidth}{XXXXXX}
\hline
Equation & $m$ & $\mathbb{E}_{p_S}[||r(x)||_2^2]$ & $\mathbb{E}_{p_S}[||r(x)||_2^2] - \mathbb{E}_{p_D}[||r(x)||_2^2]$ & $\mathbb{E}_{p_D}[||P - \hat{P}||_2^2]$ & $\mathbb{E}_{p_D}[||K - \hat{K}||_2^2]$\\
\hline
SDE & 0 & 3.6 & -0.9 & $1.02\times 10^{-1}$ & $8.8\times 10^{-3}$\\
\hline
SDE & 10 & 224.1 & 219.6 & $1.04\times 10^{-1}$ & $9.5\times 10^{-3}$\\
\hline
SDE & 50 & 1463.5 & 1459.0 & $8.73\times 10^{-2}$ & $9.1\times 10^{-3}$\\
\hline
SDE & 100 & 3986.1 & 3981.6 & $5.92\times 10^{-2}$ & $8.5\times 10^{-3}$\\
\hline
SDE & 250 & 4142.1 & 4137.6 & $3.25\times 10^{-2}$ & $7.8\times 10^{-3}$\\
\hline
SDE & 500 & 1970.2 & 1965.7 & $9.1\times 10^{-3}$ & $6.4\times 10^{-3}$\\
\hline
SDE & 1000 & 183.8 & 179.3 & $5.0\times 10^{-4}$ & $4.3\times 10^{-3}$\\
\hline
SDE & 2000 & 7.5 & 3.0 & $3.6\times 10^{-6}$ & $2.8\times 10^{-3}$\\
\hline
SDE & 4000 & 7.6 & 3.1 & $2.4\times 10^{-7}$ & $2.0\times 10^{-3}$\\
\hline

\end{tabularx}
\end{table}

\begin{table}[!htb]
\centering
\caption{Physical field reconstruction and field inversion with various number of pressure measurements (Darcy Flow, $s=256$).}
\label{tab:reconstruction_darcy_n256}
\begin{tabularx}{\textwidth}{XXXXXX}
\hline
Equation & $m$ & $\mathbb{E}_{p_S}[||r(x)||_2^2]$ & $\mathbb{E}_{p_S}[||r(x)||_2^2] - \mathbb{E}_{p_D}[||r(x)||_2^2]$ & $\mathbb{E}_{p_D}[||P - \hat{P}||_2^2]$ & $\mathbb{E}_{p_D}[||K - \hat{K}||_2^2]$\\
\hline
SDE & 0 & 953.5 & 851.5 & $4.49\times 10^{-2}$ & $2.88\times 10^{-1}$\\
\hline
SDE & 10 & 6438.5 & 6336.5 & $5.12\times 10^{-2}$ & $3.15\times 10^{-1}$\\
\hline
SDE & 50 & 37040.8 & 36938.8 & $4.29\times 10^{-2}$ & $3.14\times 10^{-1}$\\
\hline
SDE & 100 & 47121.7 & 47019.7 & $3.58\times 10^{-2}$ & $3.12\times 10^{-1}$\\
\hline
SDE & 250 & 49410.1 & 49308.1 & $2.14\times 10^{-2}$ & $3.07\times 10^{-1}$\\
\hline
SDE & 500 & 44226.5 & 44124.5 & $9.1\times 10^{-3}$ & $3.02\times 10^{-1}$\\
\hline
SDE & 1000 & 11850.1 & 11748.1 & $1.9\times 10^{-3}$ & $2.88\times 10^{-1}$\\
\hline
SDE & 2000 & 3423.6 & 3321.6 & $3.0\times 10^{-4}$ & $2.70\times 10^{-1}$\\
\hline
SDE & 4000 & 22970.3 & 22868.3 & $1.4\times 10^{-5}$ & $2.47\times 10^{-1}$\\
\hline

\end{tabularx}
\end{table}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/samples_inpaint_n16_m500_r1.png}
    \caption{Baseline data imputation on Darcy flow ($s=16$) with $m=500$ measurements.}
    \label{fig:reconstruction_darcy_base_n16}
\end{figure}

Although the reconstruction for both pressure and permeability fields improves with increasing number of samples, the physical residual is very high, particularly for smaller number of measurements. This is likely due to the incoherence between the known (measured) and unknown regions of the data samples. It is evident in Fig.~\ref{fig:reconstruction_darcy_base_n16} that the measured points do not match well with the reconstructed points. 

To reduce this discrepancy, we turn towards the idea of RePaint~\cite{}. This effectively transitions between reverse and forward steps to reduce the boundary discrepancy between measured and unmeasured regions of the data samples. At discrete time step $i$ of the reverse SDE solver, an additional $r$ \emph{resampling} steps are performed. A resampling step consists of solving the forward SDE for a single time step, followed by solving the reverse SDE for the same time step, effectively alternating $r$ times between stepping forward and stepping backward according to the SDE. This allows better mixing of the measured and unmeasured dimensions of the data, adding artificial noise before denoising, effectively incorporating more information about the known dimensions to the unknown dimensions at each resampling step. However, this comes at a significant cost: the number of function evaluations scale linearly with $r$. This can be partially alleviated by performing $r$ resampling steps only at some discrete pre-selected number of time steps instead of at each time step. However, this presents additional difficulties such as determining the optimal time steps to perform resampling at. 

\begin{table}[!htb]
\centering
\caption{Physical field reconstruction with RePaint (Darcy Flow, $s=16$, $m=500$). Imputation performed with $r$ resampling steps at each time step.}
\label{tab:repaint_darcy_n16}
\begin{tabularx}{\textwidth}{XXXXXX}
\hline
Equation & $r$ & $\mathbb{E}_{p_S}[||r(x)||_2^2]$ & $\mathbb{E}_{p_S}[||r(x)||_2^2] - \mathbb{E}_{p_D}[||r(x)||_2^2]$ & $\mathbb{E}_{p_D}[||P - \hat{P}||_2^2]$ & $\mathbb{E}_{p_D}[||K - \hat{K}||_2^2]$\\
\hline
SDE & 1 & 750.7 & 746.2 & $4.9\times 10^{-3}$ & $4.3\times 10^{-3}$\\
\hline
SDE & 2 & 26.2 & 21.7 & $3.0\times 10^{-4}$ & $2.9\times 10^{-3}$\\
\hline
SDE & 3 & 8.7 & 4.2 & $3.1\times 10^{-5}$ & $3.8\times 10^{-3}$\\
\hline
SDE & 5 & 10.6 & 6.1 & $1.9\times 10^{-5}$ & $2.9\times 10^{-3}$\\
\hline
SDE & 10 & 9.6 & 5.1 & $1.7\times 10^{-5}$ & $4.8\times 10^{-3}$\\
\hline
\end{tabularx}
\end{table}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/samples_inpaint_n16_m500_r5.png}
    \caption{Data imputation on Darcy flow ($s=16$) with $m=500$ measurements and $r=5$ resampling steps.}
    \label{fig:reconstruction_darcy_repaint_n16}
\end{figure}

We investigate the power of RePainting by setting a constant number of pressure measurements ($m=500$), and solving the reverse SDE with various numbers of resampling steps. Table~\ref{tab:repaint_darcy_n16} illustrates the results of this experiment, indicating that the resampling procedure greatly improves reconstruction performance and enhances physical residuals over the baseline data imputation strategy ($r=1$). Additionally, reconstructions rapidly improve with increasing number of resampling steps. Figure~\ref{fig:reconstruction_darcy_repaint_n16} shows the result of repainting on the imputation process. When compared to the baseline imputation of Fig.~\ref{fig:reconstruction_darcy_base_n16}, reconstructions are far more accurate and less noisy. This is a direct result of reducing the boundary discrepancy using the RePainting algorithm, leading to less noisy and more accurate sampling.

An additional advantage of field reconstruction or field inversion with such score-based generative models is that of uncertainty quantification. The method is inherently uncertain. The prior is sampled from, and we solve a stochastic differential equation to obtain samples, adding noise at each time step. Thus, sampling can be performed many times for the same pressure measurements to obtain many realizations of the reconstructed fields. Such samples can then be post-processed in some way to obtain 


==> keywords.tex <==
Generative AI, Stochastic Differential Equations, Physical Consistency, Diffusion Models, Conditional Generative Modeling
